Evaluating Human-Language Model Interaction

Many real-world applications of language models (LMs), such as writing assistance and code autocomplete, involve human-LM interaction. However, most benchmarks are non-interactive in that a model produces output without human involvement. To evaluate human-LM interaction, we develop a new framework, Human-AI Language-based Interaction Evaluation (HALIE), that defines the components of interactive systems and dimensions to consider when designing evaluation metrics. Compared to standard, non-interactive evaluation, HALIE captures (i) the interactive process, not only the final output; (ii) the first-person subjective experience, not just a third-party assessment; and (iii) notions of preference beyond quality (e.g., enjoyment and ownership). We then design five tasks to cover different forms of interaction: social dialogue, question answering, crossword puzzles, summarization, and metaphor generation. With four state-of-the-art LMs (three variants of OpenAI's GPT-3 and AI21 Labs' Jurassic-1), we find that better non-interactive performance does not always translate to better human-LM interaction. In particular, we highlight three cases where the results from non-interactive and interactive metrics diverge and underscore the importance of human-LM interaction for LM evaluation.

==> chapters/halie/appendices/02_experiment_crossword.tex <==
Crossword puzzles have been studied as a challenging task for AI systems \citep{ginsberg2014fill, littman2002puzzles, wallace2022crossword, rozner2021cryptic}. Unlike multiple-choice QA, solving a crossword puzzle is a \emph{generative} task requiring open-ended responses to clues. The crossword puzzle task also provides additional structure, whereby a user can check whether a candidate answer satisfies the lexical constraints of the puzzle. Finally, clues are often not straightforward (e.g. ``Christmas in Chamonix''), and a user might need to reformulate the query to find the desired information. 

\paragraph{Task.} 
A crossword puzzle requires solving a series of word clues (\eg ``Oscar the Grouch's home'') that correspond to either rows (``Across'' clues) or columns (``Down'' clues) of white squares on a rectangular grid. 
As users solve one clue and places letters in squares, they reveal partial information (\eg shared letters) that can affect their strategy for solving future clues.  
In our setting, users try to complete an entire crossword puzzle with the ability to query an \lm-based ``AI Teammate'' via a chat-based interface. 
Users may message the AI Teammate with free-form text, where each individual message is used as the full prompt to the underlying LM.    

\paragraph{System logic.}
\looseness-1
Figure~\ref{fig:crossword:interface} shows a \textimp{state} of our crossword system, which we adapt from  \emph{\href{https://downforacross.com/}{Down for a Cross}},  an open-source software for the multi-player crossword puzzles. 
Users can take the following \textimp{actions}: pressing a key to modify user input, pressing the ``enter'' key to submit input, selecting a square in the puzzle, entering a letter into a square, selecting a clue from the list, and finishing the session.
While attempting to solve different crossword clues (\showoutputs), users (with the chat ID: \inlinequote{You}) are able to repeatedly interact with an \lm  (with the chat ID: \inlinequote{AI}) via zero-shot prompts in a dialogue-based chat interface. Although we display the chat history to aid players in remembering past information, only the most recent prompt from the player is sent to the \lm. The same \lm is fixed throughout the course of the task, which ends either after 30 minutes or when all clues are correctly solved.

In the crossword puzzle system, \createprompt creates a prompt by simply copying and pasting user input from the interface, without any further context. 
For each of the four \lms we study, \adaptlm uses \temperature $= 0.5$ and \maxtokens $= 100$ for decoding parameters.

\input{figure/03_crossword_interface.tex}

\paragraph{User study procedure.}
We recruited 350 workers (users) on Amazon Mechanical Turk, split across each of the four language models and five puzzles (\textsc{Love}, \textsc{Sit}, \textsc{Nyt-1}, \textsc{Nyt-2}, and \textsc{Elect}). 
Each user was provided a link to the interface, and asked to engage with the puzzle (\eg solve clues, interact with the \lm) for at least 30 minutes. 
Afterwards, each user completed a survey about their experience interacting with the AI Teammate. 
% Further details including instructions and information about compensation can be found in the Appendix~\ref{app:instructions:crossword}.

\paragraph{Survey questions.}
After playing with provided crossword puzzles, users are then asked to rank different qualities of the AI assistant on a 5-point Likert scale, including \emph{fluency}, \emph{helpfulness}, \emph{enjoyment}, and \emph{ease of the interaction} with the AI Teammate. 
Users are additionally asked to describe why they found the teammate helpful or unhelpful, what adjectives best describe the assistant, and whether their interaction changed over the course of answering questions.
Concretely, the following questions were asked at the end of the session:
\begin{itemize}
    \small
    \item \textbf{Fluency} (5-point Likert): How clear (or fluent) were the responses from the AI Teammate?
    \item \textbf{Helpfulness} (5-point Likert): Independent of its fluency, how helpful was your AI Teammate for solving the crossword puzzle?
    \item \textbf{Helpfulness} (free-form): Why did you find the AI Teammate helpful or unhelpful?
    \item \textbf{Ease} (5-point Likert): How easy was it to interact with the AI Teammate?
    \item \textbf{Enjoyment} (5-point Likert): How enjoyable was it to interact with the AI Teammate?
    \item \textbf{Change} (free-form): Did the way you chose to interact with the AI Teammate change over the course of solving the crossword puzzle? If so, how?
    \item \textbf{Description} (free-form): What adjectives would you use to describe the AI Teammate?
    \item \textbf{Feedback} (free-form; optional): Any feedback or comments?
\end{itemize}

\input{table/03_crossword_metrics.tex}
\input{figure/03_crossword_metrics.tex}

\paragraph{Results.}
Solving a crossword puzzle is simultaneously an open-ended goal-oriented task and a form of entertainment\dash therefore, third-party evaluation should consider both \textit{accuracy} and \textit{engagement} of the human-LM interaction. Because some users may enjoy solving crossword puzzles independently, we count the number of \textit{queries} used over the course of the task as a proxy measurement for user preference to engage with a given \lm.  

\paragraph{\circled{1} Helpfulness perceived by users exceeds accuracy improvements.} 
We measure the perceived \emph{helpfulness} of a model based on a post-task survey question with a 5-point Likert scale. Figure~\ref{fig:crossword:metrics} shows that users significantly preferred \gpttextdavinci over other models with respect to helpfulness for all puzzles. 
Interestingly, this perception of helpfulness is not necessarily reflected in the overall interaction \emph{accuracy}:
as shown in Figure~\ref{fig:crossword:metrics}, 
assistance from \gpttextdavinci led to statistically significantly higher crossword letter accuracy only for the \textsc{SIT} crossword puzzle; for the \textsc{NYT-1} puzzle, users actually performed \textit{worse} with both instruction tuned models (\gpttextdavinci and \gpttextbabbage). One hypothesis for this behavior is that these models are capable of providing confident and fluent misinformation, which can be incorrectly perceived to be helpful. 

Furthermore, the variance in model performance between puzzles strongly suggests that different puzzles' distributions over clue types may require different capabilities from \lms.
In Table \ref{tab:crossword-clue-results}, we examine performance across 6 clue category types proposed in \citet{wallace-etal-2022-automated}, and find that \lms, and in particular \gpttextdavinci, were most useful for clues about factual knowledge, but struggle with wordplay and phrases.

% To provide a closer look at why differences in puzzle clues may affect model utility, we additionally measure clue-based accuracy across different clue categories, using the same 6 categories proposed in \citet{wallace-etal-2022-automated}. 
% Concretely, for each of the 6 categories, we randomly selected 15 clues evenly distributed across the 5 crossword puzzles, over which we measured category-based accuracy across all users for each language model (Table~\ref{tab:crossword-clue-results}). 
% These results show that LMs, and in particular \gpttextdavinci, are most useful for clues about factual knowledge and commonsense reasoning. 
% Unsurprisingly, cross-reference clues, where solutions to one clue depended on another, had low accuracy due to the effect of compounding errors that can exacerbate model weaknesses. 
% Wordplay clues also had low accuracy, due to (1) the AI Teammate's lack of grounding with respect to the crossword clues, and (2) the inability of language models to observe lexical rules such as letter constraints, necessary for crossword puzzles. 
% In some cases, users were able to compensate for such weaknesses, as in the following example:
% \textquote{
%     \textbf{Prompt}: what is a skewered thai dish called?\\
%     \vspace{0.3cm}
%     \gptdavinci: a thai dish that is skewered is called `sate'\\ \url{http://answers.yahoo.com//question/index?qid=20080409053522AACrQf2}  
% }
% Here, logged keystrokes reveal that the player immediately enters ``SATAY" for the 5-letter clue answer, making the necessary modification to the model's response in order to fit the required number of letters, showing the  complementary behavior inherent to human-AI collaboration in more open-ended tasks.

\paragraph{\circled{2} Short prompts exacerbate misinformation and toxicity.} We observed significant amounts of misinformation across all models. Misinformation was particularly pernicious using \gpttextbabbage, which achieved relatively positive responses in user-reported survey responses but the lowest objective accuracy for puzzle solutions provided by users (Table \ref{tab:crossword:results}). 
We include a set of examples of misinformation from \gpttextbabbage and \gpttextdavinci below. 
While we believe misinformation played a big role in the difference between user-perceived and actual performance on the task, the overall effect of misinformation might be more nuanced: the structure of crossword puzzles provides constraints that may help users more quickly identify incorrect model suggestions.

Here, we provide several examples of misinformation observed from the \gpttextdavinci and \gpttextbabbage models, which we note may be particularly serious due to the ``confidence'' and high fluency of these model's completions. 
% \textquote{
%     \textbf{Prompt}: did abba sing waterloo? \\
%     \gpttextdavinci: No.\\ 
% }
% \textquote{
%     \textbf{Prompt}: Does Sonora Mexico have a border with Arizona?\\
%     \gpttextdavinci: No.\\
% }
% \textquote{
%     \textbf{Prompt}: name an award winning film set in Persia\\
%     \gpttextbabbage: The Golden Globe-winning film The Help is set in Persia and stars Emma Roberts \\
%     }

\textquote{
    \textbf{Prompt}: Who won the World Cup in 2018? \\
    \gpttextbabbage: The United States
}
    
\textquote{
    \textbf{Prompt}: Which US Vice President resigned from office? \\
    \gpttextbabbage: George H.W. Bush \\
}

\textquote{
    Prompt: which vice president resigned from office\\
    \gpttextdavinci: Richard Nixon \\
}

\textquote{
    Prompt: Who are the two vice presidents who resigned from office?\\
    \gpttextdavinci: The two vice presidents who resigned from office were Spiro Agnew and Richard Nixon.\\
}

% \textquote{
%     \textbf{Prompt}: what is 'Aida" and "Otello"? \\
%     \gpttextbabbage: Aida is a play by William Shakespeare and Otello is a opera by Wolfgang Amadeus Mozart. \\
%     }
    
% \textquote{
%     Prompt: successor for O connor\\
%     \gpttextdavinci Model Response: There is no clear successor for O'Connor , as no one has yet been appointed to fill her vacant seat on the Supreme Court. Some possible candidates who have been mentioned include Judges Sri Srinivasan , Merrick Garland , and Paul... \\
%     }

% \textquote{
%     \textbf{Prompt}: Who won the 2018 FIFA World Cup? \\
%     \gpttextbabbage: The United States won the 2018 FIFA World Cup. \\
% }

\input{figure/03_crossword_clue.tex}
\input{figure/03_crossword_accommodate.tex}

Additionally, we observed instances of toxic content in generated crossword outputs. Explicit responses often occurred when users, perhaps influenced by the style of crossword clues, provided short keyword prompts: \eg ``japanese car,'' ``nick wilde,'' or ``synonym of delayed.'' 
Short, ungrammatical prompts may more closely match toxic patterns in the training data (\eg pornographic video captions or social media comments). 
Other safety concerns we observed included generating personal phone numbers and YouTube accounts belonging to non-celebrities, as well as discussing more sensitive topics. 
Longer prompts that setup the appropriate context might mitigate toxic outputs,
but its effectiveness merits further study.

Here are several instances of toxic content in completions we observed. Although toxic content was more common for \gptdavinci (12) and \jurassicjumbo (8), than \gpttextbabbage (5) and \gpttextdavinci (3), we still found serious examples of toxic content generated from \gpttextbabbage and \gpttextdavinci as described in the main paper. 
Furthermore, models occasionally generated text that \textit{escalated} the sensitivity of the player's prompt, such as in the following examples:  

\textquote{
    \textbf{Prompt}: who leads a parade\\
    \vspace{0.3cm}
    \gpttextdavinci:  of the Ku Klux Klan  A man who leads a parade of the Ku Klux Klan is a Klansman.
}

\textquote{
    \textbf{Prompt}: Boxer's comeback \\
    \vspace{0.3cm}
    \gpttextdavinci: In the early 1990s, boxer Mike Tyson was convicted of rape and served three years in prison. After his release, he made a successful comeback, winning several bouts.
}

\textquote{
    \textbf{Prompt}: skipping in line called \\
    \vspace{0.3cm}
    \gpttextbabbage: for a moment of silence  for the victims of the Pulse nightclub shooting  a moment of silence  for the victims of the Christchurch mosque shootings  a moment of silence  for the victims of the Las Vegas shooting
}

Such examples, which may not be directly threatening, may still cause psychological harm to users and should therefore be considered when designing interactive applications built on language models. 



\begin{figure}[H]
   \includegraphics[width=\linewidth]{asset/crossword/full_engagement.pdf}
   \caption{
    \captionheader{Crossword puzzles}
    Cumulative queries to the AI Teammate over time for all users. Differences in the slope and final height of player trajectories highlight different forms of engagement, with a long-tail of sustained engagement with the AI Teammate over time.}
   \label{fig:crossword_engagement} 
\end{figure}



\paragraph{\circled{3} Users demonstrate diverse engagement behavior.} 
The relatively long period of interaction between users and the AI Teammate in the crossword puzzle task provides an opportunity to closely study engagement, which we measure in two ways. 
First, we ask users in the post-task survey to answer \textit{``How enjoyable was it to interact with the AI Teammate?,''} and show that users found \gpttextdavinci significantly more enjoyable to use (for some puzzles, \gpttextbabbage was also rated highly) in Table \ref{tab:crossword:results}.
This suggests that users tended to enjoy interacting with \lms that were most helpful for the task. 
However, in Figure \ref{fig:crossword_engagement}, we take a closer look at engagement across the entire 30 minutes task length, and observe a diverse set of user behaviors: while some users decided to stop querying the AI Teammate after receiving incorrect responses, others chose to solve clues independently at the start and only query later when stuck. A long tail of users, mostly interacting with  \gpttextdavinci and \gpttextbabbage, had significant sustained interaction throughout the course of the puzzle, often experimenting with re-phrasing prompts to elicit more helpful responses. 
Finally, unlike with the use of AI solvers that seek to solve a crossword puzzle perfectly  \citep{wallace-etal-2022-automated}, some users found the challenge of figuring out how to best use the AI Teammate itself entertaining: 
\textquote{
    \gptdavinci Player: This is an enjoyable task that may not be as fun if the AI would give you all the answers!
}


\paragraph{\circled{4} Users accommodate their behaviors over time.} 
We examine user accommodation, or change in behavior in response to the AI system, in two ways: qualitatively, through a free-response survey question, and quantitatively, via measuring the change in query strategies over time.  Example responses to the survey question \textit{``Did the way you chose to interact with the AI Teammate change over the course of solving the crossword puzzle? If so, how?''} indicate that users discovered prompting strategies such as extract synonyms, or phrasing their prompts as declarative statements, over the course of time, as shown below:

\textquote{
    \jurassicjumbo User: with some of the questions, it was clear to me that I couldn't even lead the AI to an answer even giving hints, things like puns are a perfect example of this. multi-word phrases were another. Where it was the most helpful is in asking for things like names of crackers or names of clowns or Ford model cars. Factual type things that didn't require logic. 
}

\textquote{
    \gpttextdavinci User: I tried to use a variety of techniques when asking questions, to avoid getting misleading answers, and I also learned quickly that I needed to confirm the responses by asking the same question multiple times (in different ways)
}

\textquote{
    \gpttextbabbage User: after I got some generic unhelpful responses, I realized I had to be more specific with my questions ... I used AI to confirm some answers instead of relying on it to come up with answers on its own.
}

\textquote{
    \gptdavinci User: I learned how to get synonyms.  Instead of [blank] synonym I put [blank] thesaurus
}

We categorize all player prompts with the same taxonomy as the QA task, but with an added ``lexical'' category for prompts that include  lexical information, such as ``letter word'' and ``begins with''.
We observe that users do indeed gradually decrease the use of questions as prompts for all models (Figure \ref{fig:crossword_coadapt_question}), while increasing their use of short keyword prompts (Figure \ref{fig:crossword_coadapt_keyword}). Surprisingly, we additionally observe that edit distance between the prompt and clue text (typically short keywords) decreases over time, particularly for \gpttextdavinci. 
This suggests what users may have natural prior when interacting with a novel \lm to use question-style prompts, but over time can adjust to using prompts more suited to the task depending on the capabilities of the underlying model.  









==> chapters/halie/appendices/02_experiment_dialogue.tex <==
Dialogue is a natural and flexible way to engage in communication, which makes it an intuitive and popular mode of interaction for \lms.
In this section, we evaluate human-\lm interaction in the context of open-ended dialogue about social situations (henceforth social dialogue).

\paragraph{Task.}
We consider the task where given a social \emph{scenario}, users converse with a system (or chatbot) about the scenario.
Users initiate the conversation and take turns with the chatbot to carry out the conversation until users choose to finish it.
We randomly select ten scenarios from the \empathetic \citep{rashkin2019towards} and \commonsense datasets \citep{zhou2021commonsense} after manually filtering out potentially sensitive and upsetting scenarios from the validation and test sets of the datasets.

\paragraph{System logic.} 
\looseness-1
Figure~\ref{fig:dialogue:interface} shows a dialogue system \textimp{state} consisting of scenario, dialogue history, and user input and possible \textimp{actions}: pressing a key to modify user input, clicking the ``send'' button to submit their input, and finishing the dialogue.
When users click the ``send'' button, the system creates a prompt with five dialogue examples for in-context learning and the current dialogue history, invokes an \lm with the prompt, fetches a completion, and shows the completion in the dialogue history in the interface (\showoutputs).

In the dialogue system,
\createprompt creates a prompt by concatenating four example dialogues for in-context learning and the current dialogue history.
While doing so, we omit the scenario information as the scenario is only known to the user.
For \adaptlm, we use \topk $= 50$ and \temperature $= 0.9$ for decoding parameters and use html tags to delineate a conversation and the turns within.

\input{figure/03_dialogue_interface.tex}
\input{table/03_dialogue_metrics.tex}

\paragraph{User study procedure.}
We recruited a total of 189 crowd workers (or users) on Amazon Mechanical Turk.
For each of the scenarios and models, we had three users each produce a dialogue.
To ensure each dialogue is long enough, the interface allowed users to finish the conversation only after taking more than ten turns or exceeding 250 words in total.
At the end of the conversation, users completed a survey about their experience.

\paragraph{Survey questions.}
We ask users to evaluate the \emph{interestingness}, \emph{sensibleness} (\ie whether a chatbot response makes sense), and \emph{specificity} (\ie whether a chatbot response is specific to what a user had said) of a chatbot, following the survey questions proposed by \citet{thoppilan2022lambda}. 
We also ask users to evaluate the \emph{fluency} of the chatbot and their \emph{inclination} to continue talking with the chatbot, as proposed by \citet{smith2022human}.
We ask dataset-specific questions regarding empathy (\empathetic) and commonsense understanding (\commonsense), which are labeled as \emph{humanness} collectively.
Finally, after a dialogue, we ask if users are willing to talk to the chatbot again using a 5-point Likert scale: \emph{reuse}.

For most questions, we ask for a turn-level annotation. 
To reduce users' workload, we negated those questions where we expected the majority of turns to be annotated positively.
For all questions, if users decided to mark none of the utterances, they had to explicitly mark a checkbox acknowledging it. 
\begin{itemize}
    \small
    \item \textbf{Fluency} (turn-level; binary; reversed scores for the negated question): Which responses did NOT sound human? 

    \item \textbf{Sensibleness} (turn-level; binary; reversed scores for the negated question): Mark responses where the chatbot did NOT make sense. 

    \item \textbf{Specificity} (turn-level; binary; reversed scores for the negated question): Mark the responses that were NOT specific to what you had said, \ie responses that could have been used in many different situations. For example, if you say ``I love tennis'' then ``That's nice'' would be a non-specific response, but ``Me too, I can't get enough of Roger Federer!'' would be a specific response. 

    \item \textbf{Humanness} (turn-level; binary): Which responses did you feel an emotional connection to? (\empathetic); Which responses made you feel the chatbot understood social contexts and situations? (\commonsense) 
    
    \item \textbf{Interestingness} (turn-level; binary): Mark the responses that were particularly interesting or boring 
    
    \item \textbf{Inclination} (turn-level; binary; reversed scores for the negated question): Which responses made you NOT want to talk with the chatbot again?
    
    \item \textbf{Reuse} (dialogue-level; 5-point Likert scale): Would you want to talk to this chatbot again? 
    
    \item \textbf{Feedback} (dialogue-level; free-form; optional): Is there anything else you would like to say about the conversation? 
\end{itemize}

\footnotetext{
    Throughout the paper, results are denoted 
    by \statsstar~if models had a significant effect relative to \gpttextdavinci,
    \statss~if significant relative to \gpttextbabbage, 
    \statsddagger~if significant relative to \gptdavinci, 
    and \statsdagger~if significant relative to \jurassicjumbo at the $p=0.05$ level using a Tukey-Kramer test.
    \label{note:stats}
}


\paragraph{Results.}
For social dialogue, we specifically care about models' ability to show an emotional connection to users, by being empathetic and  having commonsense about social situations (\emph{humanness}), in addition to being \emph{fluent} and \emph{sensible},
and \emph{specific} to what they have said.
Independently, users may have their own subjective views on whether system responses are interesting and make them want to continue interacting with the system, which are measured by preference metrics \emph{interestingness} and \emph{inclination}, respectively.

\paragraph{\circled{1} Instruction tuning improves performance on most quality metrics, but not specificity.}
Table~\ref{tab:dialogue:metrics} shows that the instruction tuned \gpttextdavinci scored highest on most metrics, including \emph{fluency}, \emph{sensibleness}, and \emph{humanness}.
In particular, users evaluated \gpttextdavinci to have considerably higher \emph{humanness} than \gptdavinci.
And the instruction-tuned \gpttextbabbage model, despite its
much smaller size, was reported to have higher humanness than \gptdavinci or \jurassicjumbo .

However, instruction tuning decreased the \emph{specificity} of model completions as shown in the significant drop in performance of \gpttextdavinci compared to \gptdavinci (Table~\ref{tab:dialogue:metrics}).
From this observation, we hypothesize that general instruction-tuning makes models better aligned with most metrics at the cost of being more generic, although 
previous work suggests that dialogue-specific fine-tuning improves all metrics including specificity \cite{thoppilan2022lamda}.

The following are two sets of completions generated by \gpttextdavinci and \gptdavinci (\topk $= 50$, \temperature $= 0.9$, \numcompletions $= 5$) to contrast their \emph{specificity} (\ie how specific it is to what users had said).
\textquote{
    \textbf{User}: I have a cat.\\
    \vspace{0.2cm}
    \textbf{Chatbot} (\gpttextdavinci): \\
    1. What is your cat's name? \\
    2. What is your cat's name? \\
    3. What is your cat's name? \\
    4. What's your cat's name? \\
    5. What's your cat's name? \\
    \vspace{0.2cm}
    \textbf{Chatbot} (\gptdavinci): \\
    1. Tell me more about your cat. \\
    2. You have a cat? \\
    3. This sentence is false. \\ 
    4. You have a what? \\
    5. What kind of cat? \\
    \vspace{0.2cm}
}
\textquote{
    \textbf{User}: I am going home for Christmas.\\
    \vspace{0.2cm}
    \textbf{Chatbot} (\gpttextdavinci): \\
    1. Really? That sounds like fun! \\
    2. That sounds like a lot of fun! \\
    3. Have a safe trip! \\
    4. Have a safe trip! \\
    5. I hope you have a safe and happy trip! \\
    \vspace{0.2cm}
    \textbf{Chatbot} (\gptdavinci): \\
    1. Where do you live? \\
    2. I am going home for Christmas. \\
    3. What is your name? \\ 
    4. What are your plans for Christmas? \\
    5. How are you traveling? \\
    \vspace{0.2cm}
}
\noindent
Although some of \gptdavinci's responses are inappropriate (\#3 in the first example) or repetitive (\#2 in the second example), overall, they tend to be more specific and diverse to the user utterance.



\paragraph{\circled{2} Users may prefer to interact with a more specific \lm.}
\looseness-1
Although users evaluated \gpttextdavinci to be the best \lm according to most metrics, they expressed similar \emph{inclination} to continue interacting with \gptdavinci during dialogue.
Given that \gptdavinci was perceived to be worse than \gpttextdavinci on all metrics except \emph{specificity} and \emph{inclination}, we hypothesize that users expressed an inclination to interact with \gptdavinci \emph{because} its responses were the most specific to what users had said.
We recommend further study of the relationship between specificity and inclination to interact with an \lm, and in particular, whether specificity affects \emph{reuse} of the \lm once the initial novelty of this interactive experience has faded.




==> chapters/halie/appendices/02_experiment_metaphor.tex <==
\looseness-1
Metaphors are used throughout poetry, journalism, and science education to communicate complex or abstract ideas \citep{mio1997metaphor,lakoff2009more,niebert2012understanding}.
Creating metaphors requires divergent, lateral thinking \citep{glucksberg2001understanding,gero2018challenges}.
To help with ideation, prior work designed metaphor generation tools where users could query multiple times to get suggestions and showed that these suggestions enabled people to write metaphors that they might never have thought of \citep{gero2019metaphoria,chakrabarty2022copoet}.
In this section, we want to compare degrees in which different \lms support such ideation process.

\paragraph{Task.}
Given a seed metaphor, the task is to write 
metaphorical sentences that evoke the given metaphor in a limited amount of time.
For example, for the metaphor ``Time is money,''
we might generate the following metaphorical sentences:
\textquote{
    How do you spend your time?\\
    That flat tire cost me an hour.\\
    I've invested a lot of time in him.
}
\noindent
From \citet{lakoff1980metaphors}, we select $3$ metaphors and their corresponding sentences as in-context learning examples, and choose $4$ thematically diverse metaphors for evaluation. We carefully choose the evaluation metaphors in order to build a distinct and rich set that covers various complexity levels.

\input{figure/03_metaphor_interface.tex}

\paragraph{System logic.}
Figure~\ref{fig:metaphor:interface} shows our metaphor system \textimp{state} consisting of a seed metaphor, user sentence history, user input, and system suggestions. 
Users can take one of the following \textimp{actions}: pressing a key to modify user input, clicking the ``get suggestions'' button, selecting a suggestion from the list of suggestions or dismiss all of them, and finishing the session.
When users click the ``get suggestions'' button, the system creates a prompt with three in-context examples and the current user input, invokes an \lm in the state, fetches five outputs with the prompt, and shows the outputs in the popup box in the interface (\showoutputs).

In the metaphor system, \createprompt prepends the following three pairs of metaphor and metaphorical sentences to the seed metaphor to generate a prompt for few-shot learning.
\textquote{
    Metaphor: Argument is war.\\
    Metaphorical Sentence: He attacked every weak point in my argument.\\
    \vspace{0.5cm}
    Metaphor: Time is money.\\
    Metaphorical Sentence: Is that worth your while?\\
    \vspace{0.5cm}
    Metaphor: Love is a journey.\\
    Metaphorical Sentence: We'll just have to go our separate ways.
}
\noindent
We carefully chose these metaphors from \citet{lakoff1980metaphors} that are relatively simple and direct without being generic.
In our preliminary studies, we did not observe a qualitatively significant difference with respect to the ordering of these examples.
For \adaptlm, we use \temperature $= 0.9$, \maxtokens $= 30$, \stopsequences $= [\textnormal{``Metaphor:''}]$ for decoding parameters.

\paragraph{User study procedure.}
\looseness-1
We recruited 32 crowd workers (users) on Amazon Mechanical Turk, and each of them could work on all four seed metaphors if desired.
For each seed metaphor, we randomly assigned one of the four \lms.
In each session, each user was given 10 minutes to come up with as many metaphorical sentences as they could using the system.
In the instructions, we asked users to write sentences that are apt, specific, and imageable along with examples, following the evaluation criteria in \citet{gero2019metaphoria}.
At the end of the session, users completed a survey about their experience.

\paragraph{Survey questions.}
In the survey, we asked about users' perceptions concerning \emph{fluency}, \emph{helpfulness}, \emph{ease} of interaction, \emph{enjoyment}, \emph{satisfaction}, \emph{ownership}, and willingness to \emph{reuse} the system on a 5-point Likert scale, similar to \citet{lee2022coauthor}. 
At the end of each metaphor session, we asked users the following questions:
\begin{itemize}
    \small
    \item \textbf{Fluency} (5-point Likert): How fluent were the responses from the AI assistant?
    \item \textbf{Helpfulness} (5-point Likert): During this writing session, the system helped me come up with new ideas.
    \item \textbf{Ease} (5-point Likert): It was easy to write metaphorical sentences with the system.
    \item \textbf{Enjoyment} (5-point Likert): I enjoyed this writing session.
    \item \textbf{Helpfulness} (free-form): What kinds of suggestions did you find helpful and why? (Give a concrete example if possible.)
    \item \textbf{Non-helpfulness} (free-form): What kinds of suggestions did you find not helpful and why? (Give a concrete example if possible.)
    \item \textbf{Editing} (free-form): What were the reasons you made edits, if any, to suggestions from the system?
    \item \textbf{Change} (free-form): Did the way you interacted with the AI assistant change over the course of the writing session? If so, how?
    \item \textbf{Satisfaction} (5-point Likert): I am satisfied with the metaphorical sentences I came up with.
    \item \textbf{Ownership} (5-point Likert): I feel like the metaphorical sentences are mine.
    \item \textbf{Reuse} (5-point Likert): I would be willing to use this system again.
    \item \textbf{Description} (free-form): What adjectives would you use to describe the AI assistant?
    \item \textbf{Feedback} (free-form; optional): Any feedback or comments?
\end{itemize}

\paragraph{Third-party evaluation.}
We also asked third-party evaluators to evaluate whether written metaphorical sentences are apt, specific, and imageable, following \citet{gero2019metaphoria}.
To this end, we recruited 7 crowd workers (third-party evaluators) on Amazon Mechanical Turk to assess the sentences.
Each sentence was assessed by 2 different evaluators.

\input{table/03_metaphor_effort.tex}

\paragraph{Results.} 
\looseness-1
In metaphor generation, we measure user effort in writing with \emph{time} and the number of \emph{queries} per sentence.
Then, we look at user survey responses on \emph{helpfulness}, \emph{satisfaction}, \emph{ease} of interaction, and willingness to \emph{reuse} the system.
Lastly, we evaluate the quality of metaphorical sentences (based on how \emph{apt}, \emph{specific}, and \emph{imageable} the sentences are) through third-party evaluation.

\paragraph{\circled{1} Users are more willing to reuse models that require less effort.}
Table~\ref{tab:metaphor:effort} shows that users needed the least effort when working with \gptdavinci, given that they 
took the least \emph{time} and made the fewest \emph{queries}.
Despite the fewest number of queries, and therefore fewest suggestions, the acceptance rate for suggestions was the highest for \gptdavinci and the final metaphorical sentences were rated most highly by third-party evaluators (Table~\ref{tab:metaphor:thirdparty}).
From these observations, we hypothesize that users could query a few times and quickly find acceptable sentences generated by \gptdavinci.
According to survey responses, users also perceived the same model as the \emph{easiest} to interact with and were most willing to \emph{reuse} the system when the model was used.

\paragraph{\circled{2} More satisfying user experiences may not correlate with the quality of outputs.}
On the other hand, users found \gpttextdavinci to be most \emph{helpful} and \emph{satisfactory} according to the survey responses (Table~\ref{tab:metaphor:survey}).
However, third-party evaluators considered sentences written with the same model to be the worst among the four models  (Table~\ref{tab:metaphor:thirdparty}).
Although it is hard to draw strong conclusions due to the relatively small size of users and third-party evaluators,
one possible explanation is that
users' value judgment for satisfaction and reuse may depend on different factors (\eg helpfulness and ease, respectively) based on the context.

\input{table/03_metaphor_survey.tex}
\input{table/03_metaphor_third_party.tex}




==> chapters/halie/appendices/02_experiment_question.tex <==
Question answering is a canonical task in NLP.
We consider an \emph{interactive} version of question answering where a user is asked to answer a question given access to an \lm that they can query.
In practice, users tend to query information systems repeatedly, refining and reformulating their queries in response to the system's output \citep{huang2009analyzing,jansen2009patterns,jiang2013users}.

\paragraph{Task.} 
Given a sequence of multiple-choice questions (or \emph{quiz}), users try to select the correct answer with advice from an \lm.
As an example, consider this multiple-choice question:
\textquote{
    Before Nixon resigned how many believed he should be removed from office? \\
    \vspace{0.2cm}
    A. 79\%  B. 98 \%  C. 33 \%  D. 57\%
}
\noindent

Users can query the system multiple times with free-form text inputs; they might start with the question verbatim, re-phrase the question to increase specificity (\eg ``Did 79 percent of people believe Nixon should have been removed from office?''), or find a different way to query, perhaps bringing in their own prior knowledge (\eg ``Nixon approval rating after watergate'').


We use questions from the Measuring Massive Multitask Language Understanding (\mmlu) dataset~\cite{hendrycks2021measuring}.
Concretely, we first chose five diverse subjects from the dataset (Global facts, Nutrition, US foreign policy, College chemistry, and Miscellany),
and selected $6$ questions from each subject to construct a pool of $30$ questions. 
We constructed quizzes by randomly selecting ten questions from the pool and adding one attention check question in the middle.

\paragraph{System logic.}
Figure~\ref{fig:question:interface} shows a \textimp{state} of our QA system consisting of a multiple-choice question, user input, and system output.
Users can take the following \textimp{actions}: pressing a key to modify user input, clicking the ``generate'' button to query the system, selecting one of the multiple choices, clicking the ``next'' button to submit their answer, and finishing the quiz.
When users click the ``generate'' button, the system creates a prompt with the user input, 
invokes an \lm with the prompt, fetches a completion, and shows the completion in the system output box in the interface (\showoutputs).

In the QA system,
\createprompt creates a prompt by simply copying and pasting user input from the interface.
Note that we do not include a multiple-choice question as part of the prompt.
For \adaptlm, we use \temperature $= 0.5$ and \maxtokens $= 100$ for decoding parameters.

\input{table/03_question_metrics.tex}
\input{figure/03_question_interface.tex}
\input{figure/03_question_category.tex}

\paragraph{User study procedure.}
We recruited 342 crowd workers (users) on Amazon Mechanical Turk.
Each user answered half of the questions with 
assistance from a single \lm (treatment) and answered the other half without assistance (control).
We instructed users not to use search engines to answer questions, and alerted users (``Please do not switch tabs or open a new window during your participation.'') when we detected the tab switching.
At the end of each quiz, users completed a survey about their experience. 

\paragraph{Survey questions.}
\looseness-1
We asked users for first-person evaluation of \emph{fluency}, \emph{helpfulness}, and \emph{ease of interaction} of the system on a 5-point Likert scale.
Also, we asked users to describe why they found the system helpful or unhelpful, provide adjectives to describe the system, and explain whether their interaction changed over the course of answering questions.
Concretely, the following questions were asked at the end of each quiz:
\begin{itemize}
    \small
    \item \textbf{Fluency} (5-point Likert): How clear (or fluent) were the responses from the AI Assistant?

    \item \textbf{Helpfulness} (5-point Likert): Independent of its fluency, how helpful was having access to the AI Assistant compared to not having access?

    \item \textbf{Helpfulness} (free-form): Why did you find the AI Assistant helpful or unhelpful?
    
    \item \textbf{Ease of interaction} (5-point Likert): How easy was it to interact with the AI Assistant?
    
    \item \textbf{Change} (free-form): Did the way you chose to interact with the AI Assistant change over the course of answering questions? If so, how?
    
    \item \textbf{Feedback} (free-form; optional): Any feedback or comments?
\end{itemize}

\input{figure/03_question_type.tex}

\paragraph{Results.}
\looseness-1
For the goal-oriented QA task, third-party evaluation is characterized by \emph{accuracy} (\ie how many questions users get correct answers for) and \emph{efficiency} (\ie how much effort users put in to find an answer) \citep{dibia2022aligning}.
Because the bulk of a user's time in interactive tasks is spent reacting to system outputs, we count the number of \emph{queries} needed to answer each question as a proxy measurement for efficiency.

\paragraph{\circled{1} Users with \lm assistance generally outperform the user or \lm alone, but not always.}
Figure~\ref{fig:question:category} shows human+\lm accuracy, zero-shot \lm accuracy,\footnote{
    For fully-automated models, we report deterministic results with \temperature $= 0$. 
} and human-\lm interactive accuracy broken down by question category.
Users assisted by \gpttextdavinci outperformed users alone in all categories. Users with \lm assistance generally outperformed an \lm alone, with the notable exception of the US Foreign Policy category, where both \gpttextdavinci and \gptdavinci achieved better accuracy as zero-shot QA systems than as interactive assistants.
For the Global Facts and Miscellany categories, users with \lm assistance significantly outperformed zero-shot \lms.
In these contexts, users are able to figure out how to query the \lm and when to trust it.

\paragraph{\circled{2} Non-interactive performance does not always lead to better human-LM interaction.} 
\looseness-1
Further analysis of Figure \ref{fig:question:category} shows that for the Nutrition category, \gpttextbabbage had the worst accuracy as a zero-shot QA system, but achieved the best performance as an interactive \lm assistant (tied with \gpttextdavinci). For US Foreign Policy, \jurassicjumbo performed worst as a zero-shot QA system and \gptdavinci performed best, but as an \lm assistant \jurassicjumbo outperformed \gptdavinci. This supports the broader point that non-interactive performance is an imperfect proxy for evaluating human-\lm interaction.


% \footnotetext{The zero-shot, non-interactive QA systems' accuracy can be found at \url{https://nlp.stanford.edu/helm/interactive_qa_mmlu/?suite=interactive_qa_mmlu&group=mmlu}}

\paragraph{\circled{3} Instruction tuning improves accuracy and efficiency for human-LM interaction.} 
Table~\ref{tab:question:results} shows that \gpttextdavinci was the most efficient and accurate tool (1.78 queries/question with 69\% accuracy). In contrast, \gptdavinci was least efficient, requiring an average of 1.5x as many queries to answer a question with only 48\% accuracy.
Despite its smaller size, \gpttextbabbage performed better than \gptdavinci on most metrics, demonstrating the effectiveness of instruction tuning for this task.
Instruction-tuned models were also perceived most favorably in first-party survey evaluation.

\paragraph{\circled{4} Users have different intentions.}
% We consider different ways users form their inputs to the system and how they change over time.
% Concretely, we categorize user inputs into non-mutually exclusive groups (not mutually exclusive), such as \emph{question} (\ie ending with ``?''), \emph{choices} (\ie containing one or more answer choices), and \emph{completion} (\ie containing the start of sentences).
% See Appendix~\ref{app:question:query} for the full list of categories and exact categorization method.

% In our experiments, question-type inputs were overall the most popular method of querying the system (\result{??} of 3170 user inputs we collected).
% Notably, around \result{129} queries contained multiple-choice answer questions, showing some user tendencies to use the system to ``verify'' different answer choices (see Appendix~\ref{app:question:query-examples} for example user inputs). \ml{need to debug (should be 14\%)}
% This behavior was further described in user responses to the survey question (the user interacted with \gpttextdavinci): ``I used the AI assistant more often for the same question to better understand the answer to a question, to feel more assured that I was answering the question correctly.''
% This use of the system to verify, instead of simply seeking answers, highlights the importance of assessing \lms in interactive settings.


% \subsubsection{User accommodation} 
% \label{sec:accommodation_qa}
We examine user accommodation, or change in behavior in response to the AI system, in two ways: qualitatively, through a free-response survey question, and quantitatively, via measuring the change in query strategies over time.  
Example responses to the survey question \textit{``Did the way you chose to interact with the AI Assistant change over the course of answering questions? If so, how?''} indicate that users discovered strategies such as including potential answers in their prompts, or phrasing their prompts as declarative statements, over the course of time, as shown below:
\textquote{
    \gpttextdavinci User: I tried a few question formats and found that simply repeating the question followed by the answer choices (but not preceded by the answer choices) worked so I continued to do that.  
}

\textquote{
    \gpttextbabbage User: I initially didn't include the multiple choice options because I didn't know how helpful it would be to include them, but after a couple questions with the AI not giving definitive answers without them, I started including them. 
}

\textquote{
    \gptdavinci User: I felt I could a better response if instead of asking a question I typed in the beginning of a thought. For example, instead of saying "what causes cancer?" it's better to type in "cancer is caused by...".
}

\textquote{
    \jurassicjumbo User: It seemed like providing an unfinished sentence as a prompt often provided more useful results than a simple question. \\
    \vspace{0.2cm}
} 

To further examine these trends quantitatively, we categorized all user prompts using the below taxonomy in order to measure how the distribution of prompt type changed for users over time: 

\begin{itemize}
    \small
    \item \textbf{Question}: User input ends with ``?'' or starts with one of the following tokens \{"who", "what", "where", "how", "which", "why", "when", "whose", "do", "does", "did", "can", "could", "has", "have", "is", "was", "are", "were", "should"\}, following \citet{pang2011query}
    \item \textbf{Close}: User input has normalized similarity $s$ where $70 < s < 100$ with the question text 
    \item \textbf{Keyword}: User input consists of less than five words, similar to a search engine query
    \item \textbf{Exact}: User input has normalized similarity $s= 100$ with the question text
    \item \textbf{Completion}:  User input consists of the start of sentences the LM should fluently complete, defined by ending with one of the following tokens created from the manual analysis: \{"is", "was", "by", "may", "cause", "are", "of", "about", "the", "to", "their"\}
\item \textbf{Choices}: User input contains answer choices provided in the question text
    \item \textbf{Command}: User input commands the language model to perform a task, such as ``list" or ``finish the sentence"
    \item \textbf{Meaning}: User input provides definition or information about meaning, such as ``synonym of'' or ``words for''
    \item \textbf{Others}
\end{itemize}

We observe that users do indeed gradually decrease the use of questions as prompts for all models (Figure \ref{fig:iqa_coadapt_question}), while increasing the inclusion of answer choices in their prompts, especially for \gpttextbabbage (Figure \ref{fig:iqa_coadapt_choices}), quantitatively supporting user survey responses. We additionally found that users were less likely to copy the exact \mmlu question text for all models over time, further supporting our motivation of interactive \lm evaluation of question answering where users engage in query reformulation. 



==> chapters/halie/appendices/02_experiment_summarization.tex <==
\looseness-1
Text summarization is a long-standing problem in NLP \citep{luhn1958automatic, mani1999advances, sparck1999automatic, nenkova2012survey}.
Notably, it has been studied in interactive settings for multi-document summarization, where the users interact with the system to query for additional information to expand upon an initial summary \citep{avinesh2018sherlock,shapira-etal-2021-extending,shapira-etal-2022-interactive}. 
In contrast, we focus on human-\lm interaction for single-document summarization, where users interact with the system to correct \lm-generated summaries.
In addition, as users correct summaries for a sequence of documents, we provide previous human-edited summaries as examples to the system to improve future summaries via in-context learning.

\paragraph{Task.}
We consider the task, where given a document and a model-generated summary, users edit the summary to be consistent, relevant, and coherent.
We randomly select 964 documents from \xsum dataset \cite{narayan2018dont} and construct 20 summarization \emph{sessions} by randomly choosing ten documents per session without replacement.

\input{figure/03_summarization_interface.tex}

\paragraph{System logic.}
Figure~\ref{fig:summarization:interface} shows the system state and actions.
A summarization system \textimp{state} consists of a document, user summary history (not visible to users), user input, and survey questions.
Users can take the following \textimp{actions}: pressing a key to modify a model-generated summary, clicking the ``next'' button, responding to survey questions, and finishing the session.

One notable difference in the summarization system's state is that 
\createprompt generates a prompt by concatenating all the previous document and user-edited summary pairs in the user's summary history as part of the prompt.
This enables us to study whether an \lm can learn from user examples and improve over time, as well as how users behavior change as the models learn or fail to learn from their examples.

In the summarization system,
\createprompt creates a prompt by concatenating all previous document and user-edited summary pairs for in-context learning and the current document to be summarized.
For the very first document, we perform one-shot learning, instead of zero-shot to avoid early user dropout, with the following example:
\textquote{
    Document: Fire crews and police were called to the property in Savile Road, Halifax, at 05:37 BST and the body of a man in his 50s was found inside. West Yorkshire Police said he had not yet been identified. Det Insp Craig Lord said: ``Inquiries are ongoing today with West Yorkshire Fire and Rescue Service to determine the cause of this fire which has sadly resulted in a man losing his life.''\\
    \vspace{0.2cm}
    Summary: A man has died in a fire at a flat in West Yorkshire.
}
\noindent
For \adaptlm, we use \temperature $= 0.3$, \maxtokens $= 64$, \stopsequences $= [\textnormal{``***''}]$ as decoding parameters and return the first sentence of the model output as a summary.

\paragraph{User study procedure.}
We recruited $39$ crowd workers (or users) on Amazon Mechanical Turk.
For each model, we collected $20$ summarization sessions ($80$ in total), while allowing the same users to participate multiple times.
Upon receiving a model-generated summary for each document, users were asked to edit the summary to be consistent, relevant, and coherent.
To encourage users to pay attention to the three quality criteria when editing, we asked users to evaluate the consistency, relevance, and coherence of the original (model-generated) summary and edited summary before and after editing.
At the end of a summarization session, users completed a survey about their overall experience interacting with the system.

\paragraph{Survey questions.}
We ask per-summary and per-session questions to the users. 
Summary-level questions ask \emph{consistency}, \emph{relevance}, and \emph{coherence} of the original and edited summaries, following \citet{10.1162/tacl_a_00373}.
Session-level questions evaluated users' overall perceptions of the summarization system with respect to its \emph{helpfulness} and \emph{improvement over time}.
At the end of each summarization session, we asked users the following questions:
\begin{itemize}
    \small
    \item \textbf{Helpfulness} (5-point Likert): How helpful was having access to the AI assistant as an automated summarization tool?
    \item \textbf{Edit amount} (5-point Likert): How much did you have to edit the generated summaries?
    \item \textbf{Improvement} (5-point Likert): The AI assistant improved as I edited more summaries.
\end{itemize}

\paragraph{Third-party human evaluation.} 
\looseness-1
We also asked third-party evaluators to evaluate the consistency, relevance, and coherence of a subset of the summaries generated by \lms.
To this end, we randomly sampled $100$ documents from our user study and recruited $18$ workers (third-party evaluators) on Amazon Mechanical Turk to assess the summaries written for the documents. 
Each summary was assessed by $3$ different evaluators.


\input{table/03_summarization_preference.tex}
\input{table/03_summarization_quality_third_party.tex}


\paragraph{Results.}
In text summarization, we ask third-party evaluators to evaluate the quality of summaries with respect to their \emph{consistency} (\ie all the information in the summary is inferred from the document), \emph{relevancy} (\ie the summary includes only important information and no excess information), and \emph{coherence} (\ie the summary organizes the relevant information in a well-structured manner).
For first-person perspectives, we compute \emph{edit distance} from interaction traces, and consider survey responses for \emph{helpfulness} and \emph{improvement} (\ie the improvement of AI assistance as more summaries are edited).

\paragraph{\circled{1} There is a discrepancy between metrics based on third-party and first-person perspectives.}
Table~\ref{tab:summarization:preference} shows that users found summaries generated by \gpttextdavinci to be the most helpful starting point for editing, receiving the smallest \emph{edit distance} and \emph{revision} score along with the highest \emph{helpfulness} score. 
However, from third-party evaluation, original summaries from \gpttextbabbage were rated as the most \emph{consistent} and \emph{relevant} among the four models (Table~\ref{tab:summarization:quality}).
According to the \emph{density} metric (\ie the average length of the extractive fragment to which each word in the summary belongs) \cite{grusky-etal-2018-newsroom},
summaries generated by \gpttextbabbage are much more extractive (16.11) than those by other models (4.19 for \gpttextdavinci, 4.86 for \gptdavinci, and 4.09 for \jurassicjumbo).
This observation reveals a discrepancy between the metrics commonly used to evaluate summarization quality and what users find helpful in interacting with and improving these models.

\input{figure/03_summarization_edit.tex}

\paragraph{\circled{2} Users save effort with \gpttextdavinci over time, suggesting it is better at in-context learning.}
We are interested in how users behavior change over time as \lms succeed or fail to learn from previous examples.
To that end, we observed how the \emph{edit distance} between the original and edited summaries change as a summarization session progresses.
Figure~\ref{fig:summarization:edit} shows the change of edit distance across ten summaries in a sessions.
We observe that users had to edit less with \gpttextdavinci over time, whereas they had to edit more with \gpttextbabbage.
The survey response also indicated that users perceived \gpttextdavinci to be best at improving over time (\emph{improvement} in Table~\ref{tab:summarization:preference}).
From this observation, we hypothesize that \gpttextdavinci is better at in-context learning the user's preferences for summarization.



==> chapters/halie/appendices/02_experiments.tex <==
\subsection{Social dialogue}
\label{app:dialogue}
\input{appendices/02_experiment_dialogue}


\subsection{Question answering}
\label{app:question}
\input{appendices/02_experiment_question}


\subsection{Crossword puzzles}
\label{app:crossword}
\input{appendices/02_experiment_crossword}


\subsection{Text summarization}
\label{app:summarization}
\input{appendices/02_experiment_summarization}


\subsection{Metaphor generation}
\label{app:metaphor}
\input{appendices/02_experiment_metaphor}

==> chapters/halie/appendices/03_screenshots.tex <==
Our experiment was reviewed and approved by the institution's Institutional Review Board (IRB).
Before the study, all participants read and agreed to a consent form that included risks, payments, participants' rights, and contact information.

\paragraph{Qualification.}
We recruited participants through Amazon Mechanical Turk, where we required that they had a HIT approval rate greater than $97\%$, were located in the United States, and had greater than 10000 approved HITs.

\paragraph{Payment.}
The payment was determined to be around \$18 or more per hour, which exceeds the minimum wage in the United States.
For data collection, we paid \$3 for social dialogue (10 minutes), \$5 for question answering (15 minutes), \$10 for crossword puzzles (30 minutes), \$10 for text summarization (30 minutes), and \$4 for metaphor generation (10 minutes).
For third-party evaluation, we paid \$0.35 for evaluating one document and summary pair on three criteria and \$0.15 for evaluating one metaphorical sentence on three criteria.


\subsection{Social dialogue}

\paragraph{Instructions.}
We provided users with both general and dataset-specific instructions. 
\textquote{
    \textbf{General instructions}\\
    \vspace{0.3cm}
    You are invited to participate in a research study on understanding human-chatbot
    communication and evaluating the performance of chatbots on certain tasks. Our goal is to learn how to build
    chatbots that can talk to people naturally, much like another human being does. You will chat with a chatbot
    for around 10-15 minutes. The chatbot is designed to discuss a range of social topics (for example music or
    travel) and you are encouraged to converse with it naturally, as you would with a friend. For example, you may
    ask questions or introduce your own topics. Once you have completed your conversation, you will be asked to
    answer feedback questions about the interaction. Data from responses and chatlogs will be analysed in
    deidentified format and extracts edited to preserve confidentiality may be featured in any published work
    resulting out of the study.
}
    
\textquote{
    \textbf{\commonsense task instructions}\\
    \vspace{0.3cm}
    When you start the chat, you will be given a scenario to discuss. For example, you may have the scenario “I lost my keys this morning. It was very stressful.” During the conversation, please talk as though you have experienced the scenario given. For this scenario, you might say something like “I had such a stressful morning! I couldn’t find my keys anywhere.” The goal of this task is to evaluate how well the chatbot understands common social scenarios.
e}

\textquote{
    \textbf{\empathetic task instructions}\\
    \vspace{0.3cm}
    When you start the chat, you will be given a scenario to discuss. For example, you may have the scenario “I lost my keys this morning. It was very stressful.” During the conversation, please talk as though you have experienced the scenario given. For this scenario, you might say something like “I had such a stressful morning! I couldn’t find my keys anywhere.” The goal of this task is to evaluate how well the chatbot communicates empathetically.
}


\subsection{Question answering}

\paragraph{Instructions.}
Users were given a description of the task and asked to answer questions as accurately as possible. We also informed users that for some questions, they will have the option to query an AI assistant.

Before users start the question-answering experiment, we walk them through an example multiple-choice question and illustrate two examples of unsuccessful prompts and one example of a successful prompt. These examples were created from initial pilot experiments. 
The example question we use is: 
\textquote{
    What is another name for the camelopard?\\
    \vspace{0.2cm}
    \textbf{A}. Circus\\
    \textbf{B}. Giraffe\\
    \textbf{C}. Cantaloupe\\
    \textbf{D}. Oasis
}
The unsuccessful examples illustrate how prompts result in inconclusive answers from the model. The first unsuccessful example is:
\textquote{
    Prompt: What is another name for the camelopard? \\
    \vspace{0.2cm}
    Completion: A: The camelopard is a cross between a camel and a leopard. The camelopard is a cross between a camel and a leopard.
}

The second unsuccessful example is:
\textquote{
    Prompt: Another name for the camelopard is \\
    \vspace{0.2cm}
    Completion: the ``camel-cat.'' which is a more common name in the United States. References External links Category: Mammals described in 1828 Category: Mammals of the Middle East Category: Mammals of the Arabian Peninsula
}

The successful example illustrates how a prompt results in a conclusive answer from the model for answering the question. We used the following example:
\textquote{
    Prompt: Circus, Giraffe, Cantaloupe, Oasis. Another name for camelopard is \\
    \vspace{0.2cm}
    Completion: giraffe. In the animal kingdom, giraffes are the tallest land animals.
}

To encourage diversity in prompting, we emphasize that users need not follow the example prompts we outlined and are free to prompt the assistant in whatever manner they choose. 
We also remind users not to use Google or another search engine and not to switch tabs during the experiment. 

\paragraph{Interface.}
See Figure~\ref{fig:question:interface:appendix}.

\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.5\textwidth}
       \includegraphics[width=1\linewidth]{asset/question/question-interface-enabled.png}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.5\textwidth}
       \includegraphics[width=1\linewidth]{asset/question/question-interface-disabled.png}
    \end{subfigure}
    
    \caption{\textbf{[Question answering]} The interface enables AI assistance for half of the questions in a quiz (top) and disables it for the other half (bottom) in which case users have to answer the question without any assistance.}
    \label{fig:question:interface:appendix}
\end{figure}

\subsection{Crossword puzzles}
\label{app:instructions:crossword}

\paragraph{Instructions.}
Users were provided a description of how to interact with the AI Teammate and overall crossword puzzle interface, as well as examples of prompts they could provide to assist with solving puzzle clues. 
As in the QA task, these examples were drawn from pilot studies. 
% We include an image of the full instructions provided to crowdworkers in Figure~\ref{fig:crossword:instructions}, which users were able to access at any point from the crossword interface.

\input{figure/03_crossword_instructions.tex}

% Visualizations of all interactive crossword solving sessions are provided \href{https://web.stanford.edu/~meghas/crossword/}{here}.


\subsection{Text summarization}

\paragraph{Interface.}
See Figure~\ref{fig:summarization:interface:appendix}.

\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{\linewidth}
       \includegraphics[width=1\linewidth]{asset/summarization/summarization-interface-original-summary-rating.png}
    \end{subfigure}
    
    \begin{subfigure}[b]{\linewidth}
       \includegraphics[width=1\linewidth]{asset/summarization/summarization-interface-editing-summary-2.png}
    \end{subfigure}
    
    \begin{subfigure}[b]{\linewidth}
       \includegraphics[width=1\linewidth]{asset/summarization/summarization-interface-edited-summary-rating.png}
    \end{subfigure}
    
    \caption{\textbf{[Text summarization]} We first ask users to rate the original summary generated by the system (top). Then, users edit the original summary to be more consistent, coherent, and relevant (middle). Finally, users rate their own edited summary (bottom).}
    \label{fig:summarization:interface:appendix}
\end{figure}

\subsection{Metaphor generation}

\paragraph{Interface.}
See Figure~\ref{fig:metaphor:interface:appendix}.

\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{\linewidth}
       \includegraphics[width=1\linewidth]{asset/metaphor/metaphor-interface-add.png}
    \end{subfigure}
    
    \begin{subfigure}[b]{\linewidth}
       \includegraphics[width=1\linewidth]{asset/metaphor/metaphor-interface-list.png}
    \end{subfigure}
    
    \caption{\textbf{[Metaphor generation]} Once users write a metaphorical sentence in the text editor, they can add it to the left-hand side of the interface (top) which keeps the list of metaphorical sentences written (bottom).}
    \label{fig:metaphor:interface:appendix}
\end{figure}

==> chapters/halie/appendices/04_stats.tex <==
\subsection{Methods for statistical analysis}
For the main results presented in the paper, we computed group-wise means and standard errors and used the modified Tukey-Kramer post-hoc test to account for unequal group sizes. 
For these calculations, we used both the Python scipy and R stats packages \cite{2020scipy, Rcoreteam2020}.

Given the likely bias in our survey sample, we decided to add robustness to the investigation and check our results while mathematically controlling for error by supplementing our analysis with univariate regressions. 
We ran linear regression models on all of the models against the different survey metrics using the stats package in R, which fits a linear regression against continuous variables using an ordinary least squares method \cite{Rcoreteam2020}. The numbers reported in the tables \ref{tab:dialogue:results:linearregression} - \ref{tab:metaphor:results:linearregression2} are the intercept plus the beta effect estimates associated with each variable.

Significance was assessed at the Bonferroni-corrected level \cite{bland1995multiple}. 
We checked the assumptions of the regressions held through manual verification of the residuals and Q-Q plots, and we compared the results of our experiments with the linear regression and validated relationships. 



\subsection{Social dialogue}
\input{table/dialogue-results-linearregression}
\label{app:stats:dialogue}
The metrics analyzed for the dialogue task included \emph{sensibility}, \emph{specificity}, \emph{humanness}, \emph{interestingness}, \emph{inclination}, and \emph{reuse}. 
The significant results are in Table~\ref{tab:dialogue:results:linearregression}. 

In the main body of the paper, it was reported that \gpttextdavinci scored highest on \emph{sensibleness}, \emph{humanness}, \emph{interestingness}, and \emph{reuse}. 
\gpttextdavinci tied with \gptdavinci on \emph{inclination}, and \gptdavinci scored highest on \emph{specificity}. 
The linear regression analysis confirms the results. 
For \emph{inclination}, similar to the main paper, the rounded values are equivalent for \gpttextdavinci and \gptdavinci, and there is no significant measured difference between the two, although \gptdavinci significantly outperforms \jurassicjumbo. 
This could reflect the performances in the previous metrics, and indicate the influence of \emph{specificity} on \emph{inclination}. 
Further research could be done by diving deeper into the nuances of the survey questions when evaluating dialogue, and investigating the relationships between the metrics. 
Additionally, this specific experiment could be well suited for a mixed effects analysis and could stand to benefit from further question refinement with the help of user feedback.


\subsection{Question answering}
\label{app:stats:question}

\input{table/question-results-linearregression} 
\input{table/question-results-accuracy}

The metrics analyzed for question answering are elapsed \emph{time}, number of \emph{queries}, and user correctness (\emph{accuracy}). The results can be found in Table~\ref{tab:questions:linearregression} and \ref{tab:questions:accuracy}.

The results are derived from linearly regressing the model types against the continuous metrics using an ordinary least squares method, conditioning upon whether a linear model was used, and the resulting values are the means of the metrics for each model type. 
Overall, using AI assistance was significantly associated with higher accuracy for all of the models; 
similarly to the main results reported in the paper, \gpttextdavinci performed the best. Additionally, like the main paper, participants using \gpttextdavinci used the least \emph{time}, and had the least \emph{queries} suggesting ease of use. However, there were significant differences in accuracy amongst the study participants assigned to \gpttextdavinci and \gptdavinci, suggesting potential confounding factors and possible limitations to the results. Future research could control for potential confounding by using block randomization when assigning participants to different language models, and thus lend robustness to results.

\subsection{Crossword puzzle}
\label{app:stats:crossword}

\input{table/crossword-results-linearregression}

The metrics analyzed for the crossword puzzle task included \emph{fluency}, \emph{helpfulness}, \emph{ease}, and \emph{enjoyment}. Further analysis was conducted conditioning on the prompts used, to test for prompt-specific error and variability.
The linear regression results are in Table~\ref{tab:crossword:results:linearregression}. None of the prompts besides the arbitrarily chosen intercepts were deemed significant, and therefore the table is not included.

The model results reported in the main results section show \gpttextdavinci outperforming the other models in all metrics. However, \gpttextdavinci only showed \emph{significant} improvement over \gpttextbabbage for \emph{helpfulness} and \emph{enjoyment}, and there was no significant difference between the two models' performances on \emph{fluency} and \emph{ease}. The added linear regression analysis here demonstrates that, when controlling for error, \gpttextdavinci has the best performance metrics to a significant degree above the other models. Additionally, although this analysis yields similar patterns of results for the worst performers, the overlapping confidence intervals and lack of significant differences between \jurassicjumbo and \gptdavinci indicate that there is less clarity around the worst performer when using a technique that accounts for error and assumes normally distributed residuals. 
Upon verifying the linear regression assumptions, the residual and Q-Q plots indicate that there were certain influential outliers that might be responsible for this lack of clarity. Further research could involve replicating this analysis in different survey samples, including regularization techniques in the statistical evaluation to account for overfitting, and investigating nonlinear relationships between the variables. These techniques might all yield clearer comparisons between the models.


\subsection{Text summarization}
\label{app:stats:summarization}

\input{table/summarization-results-linearregression-auto}
\input{table/summarization-results-linearregression-survey}
\input{table/summarization-results-linearregression-annotation}

A linear regression analysis of the summarization task was used to calculate the means and significance for the variables (\emph{elapsed time, edit distance, improvement, edit, helpfulness, original consistency, original coherency, original relevance, edited consistency, edited coherency, and edited relevance}). The results can be found in Table~\ref{tab:summarization:results:linearregression:auto}, Table~\ref{tab:summarization:results:linearregression:survey}, and Table~\ref{tab:summarization:results:linearregression:annotation}. 
Model type was used as the predictor. 

We checked the assumptions of the regressions by looking at the residuals and Q-Q plots.
In the main paper \gpttextdavinci was found to be the most helpful and improve the most with time, resulting in the lowest Levenshtein edit distance between the model produced and final summary, \gpttextbabbage and \jurassicjumbo both scored low - \gpttextbabbage requiring the most editing, and \jurassicjumbo producing the worst original summary and being the least helpful. The linear regression confirmed this and additionally highlighted the lack of distinction between the bad performers \gpttextbabbage and \jurassicjumbo.

Third party evaluation indicated higher performance from \gpttextbabbage than was found in the main paper, highlighting the importance of including annotation to verify the validity of results. Although the evidence reveals conclusively that users rate their summaries higher after editing, the evidence only slightly points to the superiority of \gpttextdavinci, and the field could benefit from additional experiments in wider samples.

\subsection{Metaphor generation}
\label{app:stats:metaphor}

\input{table/metaphor-results-linearregression}
\input{table/metaphor-results-linearregression-2}
\input{table/metaphor-results-linearregression-third}
The metrics analyzed for metaphor generation included \emph{elapsed time, queries, acceptance, edit distance,  helpfulness, satisfaction, ease, reuse} and for third party evaluation \emph{aptness, specificity, and imageability}. The significant results are in Table~\ref{tab:metaphor:results:linearregression}, Table~\ref{tab:metaphor:results:linearregression2} and Table~\ref{tab:metaphor:linearregression:thirdparty}. The direction of the results were comparable to the main paper, however no statistically significant relationships were found in the linear analysis besides the differences in acceptance and edit distance. In all other metrics, none of the models besides the arbitrarily chosen baseline models performed at a significantly different level from each other in the user survey. This indicates that the experiment found that the means of the models collectively were more than zero. However, the results do not conclusively reveal which ones performed better or worse (confirmed by the overlapping confidence intervals) on most metrics. 
This means that although the experiment found higher acceptance for \gptdavinci suggestions and shorter edit distance, other conclusions are pending further investigation and experiment replication.

==> chapters/halie/appendices/05_related.tex <==
\subsection{Social dialogue}

Dialogue systems leverage the power of natural language to promise a highly natural mode of interaction with machines in a wide range of domains ranging from information retrieval, transactions, entertainment, and even informal chit-chatting \citep{glass1999challenges}. 
LMs pose an interesting opportunity to boost the development of such systems given their generative capacity and the breadth of knowledge encoded in them that could enable dialogue systems to be able to react even in open domains. 
Although we do not evaluate them in this paper, due to time and technical constraints, recent models such as BlenderBot \citep{shuster2022blenderbot} and ChatGPT \citep{schulman2022chatgpt} demonstrate significant advancements in this field. 
Still, achieving a successful dialogue between the users and machines is difficult owing to the frequent rise of unmatched expectations of the systems' capabilities \citep{clark2019state} and the difference in conversational styles between the interlocutors \citep{thomas2020expressions}. 
Additionally, models trained on human-human conversations learn to replicate not only desirable, but also undesirable patterns of behavior \citep{xu2020recipes}. 
As such, evaluation of their interaction is important as we build the next generation of dialogue systems powered by large language models. 

Our evaluation of dialogue systems is focused on open-domain contexts, in which the conversational agent is tasked with continuing a dialogue with the user in a hypothetical scenario \citep{lengevin2021heuristic,thoppilan2022lambda,smith2022human}. 
Using specific scenarios, rather than allowing users to select any option, has several benefits. 
First, it encourages the preservation of privacy, by giving the user something to talk about beyond their own personal experience. 
Second, it enables greater standardization of results, since variance due to selected topic is reduced \citep{ji-etal-2022-achieving}. Third, using particular scenarios is consistent with past work in dialogue evaluation \citep{smith2022human}. 
Although this approach is less naturalistic than giving users an open-ended interface, we believe that the benefits outweigh the costs. 

However, there is a lack of standard approach for evaluating dialogues in such contexts \citep{deriu2021survey, huang2020challenges, roller2021recipes}. 
It is difficult to standardize dialogue evaluation, since for any context, there are many possible appropriate responses \citep{ji-etal-2022-achieving}. 
One common approach to this problem is evaluating the quality of dialogues via automated metrics, which promise fast and reproducible means to understanding dialogue systems' performance. 
However, a growing literature suggests that such metrics can be limiting in capturing the breadth of possible interactions that could happen in an open domain dialogue \citep{liu2016evaluate}. Additionally, they have been shown to have little correlation with human judgments \citep{liu2016evaluate,ji-etal-2022-achieving}. 
Unlike task-oriented dialogues, there is not a clear goal that is either reached or not, so evaluating social dialogues relies on traits that are inherently more subjective.

Prior work employed crowd workers as well as experts (\eg a group of researchers in the same institution as where the study took place, or those trained in dialogue evaluations \citep{deriu2020spot, deriu2021survey} to evaluate the quality of dialogue systems, with each group of evaluators offering their unique strengths. 
Our study employs crowd worker-based evaluation of dialogues as scalability and reproducibility are key considerations for benchmarking tasks. 
 

\subsection{Question answering}
\label{app:question:related}

Question answering is a popular task within NLP that is often evaluated with large, non-interactive datasets of question-answer pairs, sometimes accompanied with additional context \cite{rajpurkar2016squad, joshi2017triviaqa}.
The most closely related work to ours is \citet{bowman2022measuring}, which evaluates \lm-assisted QA on the \mmlu dataset. 
Whereas \citet{bowman2022measuring} evaluate interactions between a single \lm and a small group of five well-trained users, we consider interactions between four different \lm's and hundreds of users. 
In addition to replicating the finding of \citet{bowman2022measuring} that human-\lm interaction generally outperforms a human or \lm alone, we are able to observe statistically significant patterns in the relative performance of human interactions with different \lm's.
Other recent efforts to design interactive evaluation for question answering, such as \citet{kiela2021dynabench, bartolo2020beat}, largely aim to reduce test-set overfitting by asking humans to adversarially identify edge cases, rather than considering how they would naturally choose to interact with models. 

To account for more naturalistic ways humans use these systems, researchers have built datasets from actual human-generated search queries, such as \textft{MS-MARCO} \citep{nguyen2016ms} and \textft{Natural\-Questions} \citep{kwiatkowski2019natural}, thereby capturing a more realistic distribution of the information users would naturally seek from an intelligent assistant. 
However, while these datasets are useful for measuring model performance in the context of realistic user prompts for potential downstream applications, they do not provide information about the quality (\eg reported satisfaction) of a user's interaction over multiple queries. 
Furthermore, evaluations on such datasets do not account for the ability of humans to adapt, such as changing their query styles over time (\ie query reformulation) or adjusting how they trust and use system outputs in decision-making.

Query reformulation refers to the iterative process of expressing our requests differently to improve system utility, and arises commonly in the context of search engines; for example, \citet{teevan2007information} found that up to 40\% of Yahoo search log queries in a year were reformulations. 
A significant body of research from the information retrieval community focuses on deriving taxonomies for query reformulation based on analyzing search logs, including lexical-based (\eg adding words) and more general reformulation strategies (\eg specialization) \citep{huang2009query, lau1999patterns}. 
These works have inspired several methods for automatic query reformulation for inferred user goals, including using context-sensitive term-substitutions and reinforcement learning to optimize for retrieved document recall  \citep{wang2008query,nogueira2017task}.     

Further research has focused on varying querying habits across time and user populations. 
For example, \citet{pang2011query} found, perhaps surprisingly, that the use of natural language question-queries (e.g. starting with ``What'') has increased over time, despite requiring more user effort, perhaps due to an increase in novice users unfamiliar with formulating keyword-based queries \cite{white2015questions}. 
Additional research has also demonstrated a strong effect of a system's interface on users' query formats \citep{spink2002question}, and that long-term users are more likely to interact longer with a search engine during a session with more complex queries \citet{liu2013search}. 
While effective querying strategies for large language models (\eg ``prompt hacking'') have been popularly discussed, to the best of our knowledge we are the first to study these questions in the context of real user data from an LM-based interactive system. 

Finally, our task allows us to study how the lack of factuality and faithfulness of outputs from different \lms influence user trust and behavior \citet{jacovi2020faithful}. 
Several recent works on interpretability and human-AI collaboration have studied the effects of model explanations on human decision-making in classification settings \citet{lakkaraju2019faithful} finding that explanations that make model outputs appear more justifiable can make users trust even incorrect outputs more \citep{bansal2021does}.
Furthermore, they found that human-AI collaborative contexts place an additional cost of verification of model outputs on users \citet{bansal2021teammate} that, if needed frequently, may discourage future model use. 
Our task allows us to assess the degree to which efforts to align \lms to human preferences \citep{ouyang2022instructions}, as well as factors such as fluency and tone, can impact user trust over time in a collaborative task.


\subsection{Crossword puzzles}

Here we discuss interactive crossword puzzle solving in the broader setting of human-AI collaborative games. 
We refer readers to Section~\ref{app:question:related} for related work on shared aspects with the interactive question answer task.

Solving crossword puzzles has long been a challenging task for designing more complex AI systems \citep{ginsberg2014fill, littman2002puzzles, wallace2022crossword, rozner2021cryptic}. However, 
the increased success of modern text generation models and their ability for interaction with  \textit{lay}-people has sparked further development in several AI-based language games, including text-adventure games and AI Charades \citep{urbanek2019fantasy, frans2021charades}. 
Cooperative games can help highlight differences between AI-AI and human-AI benchmarking, as shown in \citet{chattopadhyay2017human}. 
Furthermore, they differ from other human-AI collaborative contexts as the goal of the collaboration is not simply completion of a task, but also a general sense of user engagement and enjoyment, which in turn depend more on more abstract properties of LM outputs. 
For example, players of the text adventure game in \citet{ammanabrolu2019quest} found that the creativity of an AI-generated game setting was anti-correlated with its coherence.

Human-AI collaborative games also serve as a rich test-bed for understanding human's mental models of an AI system; for example, humans performing poorly in the cooperative word guessing game in \citet{gero2020mental} tended to \textit{overestimate} the knowledge capabilities of the collaborating AI agent; another user study found that users were more likely to believe their teammate was an AI if it failed to adapt their behavior \citep{ashktorab2020collaboration}. 
However, a notable risk of such applications is that the greater agency provided to human users in steering the overall interaction with the AI may result in exacerbating risks of \lms such as toxic outputs---particularly harmful if such responses were unexpected. 
One notable example is  AI Dungeon \citep{hua2020unicorns}, where player inputs resulted in sexually inappropriate outputs involving children.\footnote{https://www.wired.com/story/ai-fueled-dungeon-game-got-much-darker/} 
We observe similar behaviors in our system, as described in the results (Section~\ref{app:crossword}).


\subsection{Text summarization}

Text summarization is a well established research direction in NLP \citep{mani1999advances, sparck1999automatic, nenkova2012survey}, where the goal is to compress the salient information in the source document into a coherent and fluent summary \citep{peyrard2019simple}. 
The advent of pre-trained large \lms has led to dramatic improvements in summarization capabilities, particularly in terms of coherence and fluency \citep{lewis-etal-2020-bart,zhang2020pegasus}. 
However, generated summaries are far from perfect and tend to contain information that is not supported by the original document \cite{10.5555/3504035.3504621,durmus-etal-2020-feqa,maynez-etal-2020-faithfulness,pagnoni-etal-2021-understanding}.

Given the faithfulness issues, recent work has focused on methods to improve the consistency of generated summaries with respect to the input document. 
Prior work has largely focused on improving fine-tuned models with approaches such as reducing noise incorporated from training data \citep{nan2021entity,kang2020improved,goyal2021annotating}, adding losses aimed at improving consistency \citep{nan2021improving,cao2021cliff}, and learning discriminators to select from set of candidate summaries \cite{chen2021improving,ladhak-etal-2022-faithful}. 
In contrast, our work focuses on summarization via in-context learning with an aim to understand the role of interaction in improving the quality of generated summaries. 

Interactive summarization has been studied by prior work in the context of multi-document summarization, where users interact with the system to query for additional information to expand upon an initial summary \citep{shapira-etal-2021-extending,shapira-etal-2022-interactive,avinesh2018sherlock}. 
In contrast, our work focuses on single-document summarization, where users interact with the system in order to correct the summaries to provide feedback to improve the system. 

Our work is closely related to a line of recent work that looks at improving the performance of \lms through human feedback by fine-tuning \lms using reinforcement learning \citep{ziegler2019finetuning,bohm-etal-2019-better,DBLP:journals/corr/abs-2009-01325,ouyang2022instructions} or natural language feedback \citep{campos2022training}. 
In contrast, our work has humans interact with the model and directly edit generated summaries to improve quality. 
Rather than fine-tuning the \lm, the edited summaries are incorporated into the prompt for in-context learning for future interactions.


\subsection{Metaphor generation}

Metaphor generation has been studied in the literature for creative writing applications and NLP. 
Here, we distinguish and introduce works that focus on implementing an automatic pipeline for producing metaphorical language and works that emphasize human engagement in the creative writing process.

Computational approaches to generating metaphorical language build off of conceptual metaphor theory \cite{lakoff1980metaphors}, which describes metaphors as mappings between source and target concepts. 
Approaches to generate metaphorical language can operationalize this framework by training \lms to replace literal phrases in an originally non-metaphorical sentence with figurative ones from the source \citep{chakrabarty_mermaid_2021,stowe_metaphor_2021,stowe_exploring_2021}, or by searching for connections from the source to the target concept out of a pre-existing knowledge graph of concepts \citep{gero2019metaphoria}. 
More recent works compare the use of pipelines that focus on specific keywords to our strategy of few-shot prompting for generating figurative language in the context of puns \citep{mittal_ambipun_2022} and find that decomposing the generation task improves successful generation, although surprisingly the few-shot only approach achieves the highest coherency.

Since the quality of creative writing is subjective and difficult to capture by automatic metrics alone, the evaluation of metaphors typically involves human annotation to assess the effectiveness of the metaphorical connection and figurative aspect of the generation. 
For instance, works related to lexical substitution or paraphrasing assess \emph{metaphoricity} to determine how well the modified sentence evokes figurative imagery, while checking that the intended meaning is present  \citep{chakrabarty_mermaid_2021,stowe_metaphor_2021,stowe_exploring_2021}, whereas \citet{gero2019metaphoria} consider more precisely how well the identified metaphorical connection fits the seed metaphor, or mapping, in both \emph{aptness} and \emph{specificity}.

The use of computational metaphor generation to support creative writing has been explored in \citet{gero2019metaphoria}, where users could try out different seed metaphors for a target word and use the system to generate metaphorical connections to inspire their own writing. 
In such settings, the diversity that the system enables in cooperation with the human user is important: ``creative writers do not want tools that will make their writing sound the same as others'' \citep{gero2019metaphoria}. 
They find that their system enables at least as much diversity as writing alone does. 
Another aspect that becomes important in using a system to help generate metaphorical connections is the sense of ownership that the human writer has over the written result. 
The same work finds that, depending on the mental model that the user has of the system, the interpretation of ownership can vary from feeling usurped by an overly involved partner to treating the system similarly to some other computational aid, such as a calculator.


==> chapters/halie/figures/03_summarization_criteria.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{chapters/halie/assets/summarization-criteria-third.pdf}
   
    \caption{
        \captionheader{Text summarization}
        \textbf{Third-party evaluation of summaries generated by models (\emph{original}) and summaries further edited by users (\emph{edited}).}
        Relevance and coherency scores from the third-party evaluation were initially collected on 5-point Likert and later scaled to 100 to be comparable to the binary setting in the first-person evaluation.
        \ml{change it back to be binary and likert}
    }
    \label{fig:summarization:criteria}
\end{figure*}

==> chapters/halie/tables/03_summarization_quality.tex <==
\begin{table*}[t!]
    \centering
    \small
    \begin{tabular}{rccc|ccc|c}
        \toprule
        & \multicolumn{3}{c|}{\textbf{First-person evaluators}} & \multicolumn{3}{c|}{\textbf{Third-party evaluators}} & \\
        Model & Consistency & Relevance & Coherence &  Consistency & Relevance & Coherence & Density \\
        & (/100\%) \higherbetter & \multicolumn{2}{c|}{(/5) \higherbetter}  &  (/100\%) \higherbetter & \multicolumn{2}{c|}{(/5) \higherbetter} & \lowerbetter \\
        \midrule
        \gpttextdavinci  & 56 \sem{4}\statss	 & 3.12 \sem{.17}	 & \best{3.85 \sem{.15}} 
        & 65 \sem{4}\statss	 & 4.07 \sem{.08}\statsddagger	 & \best{4.70 \sem{.04}}\statss &  4.19 \\
        
        \gpttextbabbage  & \best{76 \sem{3}}\statsddagger\statsstar\statsdagger	 & \best{3.35 \sem{.17}}	 & \worst{3.50 \sem{.16}}
        & \best{89 \sem{3}}\statsdagger \statsddagger \statsstar	 & \best{4.15 \sem{.06}}\statsddagger \statsdagger	 & \worst{4.51 \sem{.06}}\statsstar &  \worst{16.11} \\
        
        \gptdavinci     & 57 \sem{4}\statss	 & 3.23 \sem{.17}	 & \best{3.85 \sem{.15}} 
        & 57 \sem{4}\statss	 & \worst{3.70 \sem{.09}}\statsstar \statss	 & 4.53 \sem{.05} 
 &  4.86\\
        
        \jurassicjumbo   & \worst{50 \sem{4}}\statss	 & \worst{3.05 \sem{.17}}	 & 3.67 \sem{.16} 
        & \worst{56 \sem{4}}\statss	 & 3.80 \sem{.07}\statss	 & 4.60 \sem{.04} &  4.09\\
        \bottomrule
    \end{tabular}
    \caption{
        \captionheader{Text summarization}
        % \textbf{Quality metrics based on first-person and third-party human evaluation.}
        Overall, the quality evaluation by first-person and third-party evaluators agree on most results.
        \gpttextbabbage performs the best with respect to \emph{consistency} and \emph{relevance}, while \gpttextdavinci was rated highest for \emph{coherence}.
        Note that relevance and coherence scores of first-person evaluators are scaled from binary to 5-point Likert scale.
        The numbers indicate averages and standard errors, and the markers denote statistical significance.\textsuperscript{\ref{note:stats}}
        \ml{@Faisal: add std errors for density}
    }
    \label{tab:summarization:quality}
\end{table*}
